EmbedDistill: A Geometric Knowledge Distillation for Information Retrieval

Large neural models (such as Transformers) achieve state-of-the-art performance for information retrieval (IR). In this paper, we aim to improve distillation methods that pave the way for the resource-efficient deployment of such models in practice. Inspired by our theoretical analysis of the teacher-student generalization gap for IR models, we propose a novel distillation approach that leverages the relative geometry among queries and documents learned by the large teacher model. Unlike existing teacher score-based distillation methods, our proposed approach employs embedding matching tasks to provide a stronger signal to align the representations of the teacher and student models. In addition, it utilizes query generation to explore the data manifold to reduce the discrepancies between the student and the teacher where training data is sparse. Furthermore, our analysis also motivates novel asymmetric architectures for student models which realizes better embedding alignment without increasing online inference cost. On standard benchmarks like MSMARCO, we show that our approach successfully distills from both dual-encoder (DE) and cross-encoder (CE) teacher models to 1/10th size asymmetric students that can retain 95-97% of the teacher performance.

==> 040_embedding.tex <==
%

\vspace{-2mm}
\section{Embedding-matching based distillation}
\label{sec:embed_distill}
\vspace{-1.5mm}
{Informed by our analysis of teacher-student generalization gap in Sec.~\ref{sec:theory}, we propose \embd~-- a novel distillation method that explicitly focuses on aligning the embedding spaces of the teacher and student.}
%Since modern neural IR models are inherently embedding-based, we propose to explicitly align the embedding spaces of the teacher and student via a novel distillation method, namely \embd. %Note that 
Our proposal goes beyond existing distillation methods in the IR literature that only use the teacher scores. Next, we introduce \embd~for two prevalent settings: (1) distilling a large DE model to a smaller DE model;
% \todoasr{Maybe remove this footnote to save space?}
\footnote{
CE to CE distillation is a special case of this with classification vector $w$ (cf.~Eq.~\eqref{eq:ce-desc}) as trivial second encoder.
% We  focus on DE to DE distillation setup as the CE to CE distillation is special case of the former with the classification vector $w$ (cf.~Eq.~\eqref{eq:ce-desc}) being the trivial second encoder.
} 
and (2) distilling a CE model to a DE model.
% The main contribution of this work is to propose novel distillation mechanisms for IR that go beyond simply utilizing the teacher model scores. Noting that modern neural %architectures utilized in 
% IR models are inherently embedding-based, we propose to explicitly align the embedding spaces of the teacher and student models during distillation. Next, we describe the proposed embedding matching-based distillation for two prevalent distillation setups: (1) distilling a large DE model to a smaller DE model;\footnote{We  focus on DE to DE distillation setup as the CE to CE distillation is special case of the former with the classification vector $w$ (cf.~Eq.~\eqref{eq:ce-desc}) being the trivial second encoder.} and (2) distilling a CE model to a DE model.

\vspace{-1mm}
\subsection{DE to DE distillation}
\label{sec:detode}
\vspace{-1mm}
Given a $(q, d)$ pair, let ${\tt emb}^{\rm t}_q$ and ${\tt emb}^{\rm t}_d$ be the query and document embeddings produced by the query encoder ${\rm Enc}^{\rm t}_{Q}$ and document encoder ${\rm Enc}^{\rm t}_{D}$ of the teacher DE model, respectively. Similarly, let ${\tt emb}^{\rm s}_q$ and ${\tt emb}^{\rm s}_d$ denote the query and document embeddings produced by a student DE model with $({\rm Enc}^{\rm s}_{Q}, {\rm Enc}^{\rm s}_{D})$ as its query and document encoders.
% % ############################
% Let $({\rm Enc}^{\rm t}_{Q}, {\rm Enc}^{\rm t}_{D})$ denote the query and document encoders of the teacher DE model. For a $(q, d)$ query-document pair, let ${\tt emb}^{\rm t}_q$ = ${\rm pool}\big({\rm Enc}^{\rm t}_{Q}(\tilde{q})\big)$ and ${\tt emb}^{\rm t}_d$ = ${\rm pool}\big({\rm Enc}^{\rm t}_{D}(\tilde{d})\big)$
% % \begin{equation}
% %     \resizebox{.89\hsize}{!}{${\tt emb}^{\rm t}_q = {\rm pool}\big({\rm Enc}^{\rm t}_{Q}(\tilde{q})\big);~{\tt emb}^{\rm t}_d = {\rm pool}\big({\rm Enc}^{\rm t}_{D}(\tilde{d})\big)$}
% % \end{equation}
% % \begin{align}
% % {\tt emb}^{\rm t}_q &= {\rm pool}\big({\rm Enc}^{\rm t}_{Q}(\tilde{q})\big); %~~\text{and} \nonumber 
% % %\\ 
% % {\tt emb}^{\rm t}_d &= {\rm pool}\big({\rm Enc}^{\rm t}_{D}(\tilde{d})\big)
% % \end{align}
% denote the query and document embeddings produced by the teacher model, respectively. 
% %\todoam{Consider defining {\tt emb} in 5.1.}
% %Recall that the teacher score $s^{\rm t}(q, d) = \langle {\tt emb}^{\rm t}_q, {\tt emb}^{\rm t}_d \rangle.$
% Similarly, let ${\tt emb}^{\rm s}_q$= ${\rm pool}\big({\rm Enc}^{\rm s}_{Q}(\tilde{q})\big)$ and ${\tt emb}^{\rm s}_d$ = ${\rm pool}\big({\rm Enc}^{\rm s}_{D}(\tilde{d})\big)$
% % \begin{flalign}
% % \text{Similarly,} && {\tt emb}^{\rm s}_q &= {\rm pool}\big({\rm Enc}^{\rm s}_{Q}(\tilde{q})\big);& %~~\text{and} \nonumber 
% % \\ 
% % && {\tt emb}^{\rm s}_d &= {\rm pool}\big({\rm Enc}^{\rm s}_{D}(\tilde{d})\big)&
% % \end{flalign}
% denote the query and document embeddings obtained by a student DE model with $({\rm Enc}^{\rm s}_{Q}, {\rm Enc}^{\rm d}_{D})$ as its query and document encoders. 
% %Note that the student score $s^{\rm s}(q, d) = \langle {\tt emb}^{\rm s}_q, {\tt emb}^{\rm s}_d \rangle.$
% % ############################
Now, \embd~optimizes the following embedding alignment losses in addition to the score-matching loss from Sec.~\ref{sec:ir-distill} to align query and document embeddings of the teacher and student:
% \vspace*{-2mm}
{%\footnotesize
\begin{align}
\label{eq:emb-loss-de2de-q}
% \hspace{-3mm}
 %\resizebox{0.9\linewidth}{!}{ $
R_{{\rm Emb}, Q}({\rm t}, {\rm s}; \SCal_n) 
% \nonumber \\ &\qquad
= \frac{1}{n}\sum\nolimits_{q \in \SCal_n} \|{\tt emb}^{\rm t}_{q}  - {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \|; %\nonumber 
\\
R_{{\rm Emb}, D}({\rm t}, {\rm s}; \SCal_n) 
% \nonumber \\ &\qquad
= \frac{1}{n}\sum\nolimits_{d \in \SCal_n} \|{\tt emb}^{\rm t}_{d}  - {\rm proj}\big({\tt emb}^{\rm s}_{d}\big) \|. \label{eq:emb-loss-de2de-d}
% $ }
% \vspace*{-5mm}
\end{align}
}%
%#################################### OLD ###############
\iffalse
Now, \embd~optimizes the following embedding alignment loss in addition to the score-matching loss from Sec.~\ref{sec:ir-distill}:
% \todoam{Square L2 norm?}
\begin{equation}
\begin{aligned}
\label{eq:emb-loss-de2de}
% &R_{\tt emb}({\tt emb}^{\rm t}; {\tt emb}^{\rm s}) 
% &R_{\tt emb}({\rm t}, {\rm s}; \SCal_n) = \frac{1}{n}\sum_{q \in \SCal_n} \|{\tt emb}^{\rm t}_{q}  - {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \| \nonumber \\
% &\qquad + \frac{1}{n}\sum_{d \in \SCal_n}\|{\tt emb}^{\rm t}_d  - {\rm proj}\big({\tt emb}^{\rm s}_d) \|,
% &R_{\rm Emb}({\rm t}, {\rm s}; \SCal_n)~=~ \frac{1}{n}\sum_{(q, d) \in \SCal_n} \Big(\|{\tt emb}^{\rm t}_{q}  - {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \| \nonumber \\
% &\qquad\qquad + \; %\frac{1}{n}\sum_{d \in \SCal_n}
% \|{\tt emb}^{\rm t}_d  - {\rm proj}\big({\tt emb}^{\rm s}_d) \|\Big),
\!R_{\rm Emb}({\rm t}, {\rm s}; \SCal_n) \!&=\! \frac{1}{n}\sum\nolimits_{(q, d) \in \SCal_n}\!\!\! \big(\|{\tt emb}^{\rm t}_{q} \! - \! {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \|
%\\ %\frac{1}{n}\sum_{d \in \SCal_n}
%&\qquad \qquad 
+ \|{\tt emb}^{\rm t}_d \!  - \! {\rm proj}\big({\tt emb}^{\rm s}_d) \|\big),
\end{aligned}
\end{equation}
where ${\rm proj}$ is an optional trainable layer that is required if the teacher and student produce different sized embeddings. %Note that the loss in Eq.~\eqref{eq:emb-loss-de2de} aims to ensure that both query and document embeddings of the teacher and student model are aligned. 
Alternatively, one can employ other variants of \embd %embedding alignment loss that only focuses on either query or document embeddings. % of the teacher and student models. 
% For example, 
, e.g., focusing on only aligning the query or document embeddings takes the following form (cf.~Fig.~\ref{fig:de2de-embed}).
%the embedding alignment that only focuses on matching query embeddings takes the following form (cf.~Fig.~\ref{fig:de2de-embed}).
% \medmuskip=0mu
% \thinmuskip=0mu
% \thickmuskip=0mu
\begin{align}
\label{eq:emb-loss-de2de-q}
% \hspace{-3mm}
 %\resizebox{0.9\linewidth}{!}{ $
R_{{\rm Emb}, Q}({\rm t}, {\rm s}; \SCal_n) 
% \nonumber \\ &\qquad
= \frac{1}{n}\sum\nolimits_{q \in \SCal_n} \|{\tt emb}^{\rm t}_{q}  - {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \|; %\nonumber 
\\
R_{{\rm Emb}, D}({\rm t}, {\rm s}; \SCal_n) 
% \nonumber \\ &\qquad
= \frac{1}{n}\sum\nolimits_{d \in \SCal_n} \|{\tt emb}^{\rm t}_{d}  - {\rm proj}\big({\tt emb}^{\rm s}_{d}\big) \|. \label{eq:emb-loss-de2de-d}
% $ }
\end{align}
\fi
%#################################### OLD ###############
%
% \subsubsection{Asymmetric DE}
% \label{sec:asymm-de2de}
%
\noindent\textbf{Asymmetric DE.}~
% Inspired by Section~\ref{sec:theory},
We also propose a novel student DE configuration where the student employs the teacher's document encoder (i.e., ${\rm Enc}^{\rm s}_{D} = {\rm Enc}^{\rm t}_{D}$) and only train its query encoder, which is much smaller compared to the teacher's query encoder.
For such a setting, it is natural to only employ the embedding matching loss in Eq.~\eqref{eq:emb-loss-de2de-q} as the document embeddings are aligned by design (cf.~Fig.~\ref{fig:de2de-embed}).

% \begin{wrapfigure}{r}{0.60\linewidth}
%     \vspace{-5mm}
%     \centering
%     \includegraphics[page=2,width=0.99\linewidth,trim=0 6cm 6cm 0,clip]{figures/TGT-Beyond Drawing.pdf}
%     % \includegraphics[page=4,width=0.95\linewidth,trim=0 6cm 8cm 0,clip]{figures/TGT-Beyond Drawing.pdf}
%     \caption{Proposed DE to DE distillation with query embedding matching. % between the teacher and student. 
%     The figure describes a setting where student employs an asymmetric DE configuration with a small query encoder and a large (non-trainable) document encoder inherited from the teacher. {The smaller query encoder ensures small latency for encoding query during inference, and large document encoder leads to a good quality document index.} % which does not significantly affect the run-time latency as the index is constructed offline. %Proposed DE$\to$DE asymmetric distillation with query embedding matching
%     }
%     \label{fig:de2de-embed}
%     \vspace{-3mm}
% \end{wrapfigure}

Note that this asymmetric student DE does not incur an increase in latency despite the use of a large teacher document encoder. This is because the large document encoder is only needed to create a good quality document index offline, and only the query encoder is evaluated at inference time.
% \manzil{while the search cost remains the same}.
Also, the similarity search cost is not increased as the projection layer ensures the same small embedding dimension as in the symmetric DE student.
Thus, for DE to DE distillation, we prescribe the asymmetric DE configuration universally. Our theoretical analysis (cf.~Sec.~\ref{sec:theory}) and experimental results (cf.~Sec.~\ref{sec:experiments}) suggest that the ability to inherit the document tower from the teacher DE model can drastically improve the final performance, especially when combined with query embedding matching task (cf.~Eq.~\ref{eq:emb-loss-de2de-q}). %the embedding matching-based distillation.

\vspace{-1mm}
\subsection{CE to DE distillation}
\label{sec:cetode}
\vspace{-1mm}
Given that CE models jointly encode query-document pairs, individual query and document embeddings are not readily available to implement embedding matching losses as per Eq.~\ref{eq:emb-loss-de2de-q} and \ref{eq:emb-loss-de2de-d}. This makes it challenging to employ \embd~for CE to DE distillation.

% \iffalse
% Let \smash{${\rm Enc}^{t}$} be the (single) teacher CE model encoder, and \smash{$({\rm Enc}^{\rm s}_{Q}, {\rm Enc}^{\rm s}_{D})$} denote the student DE model's query and document encoders. When distilling from a CE to DE model, defining an effective embedding matching task is not as straightforward as in Sec.~\ref{sec:detode}:
% % distilling between two DE models:
% since CE models jointly encode query-document pairs, it is not obvious how to extract individual query and document embeddings for matching. 
% \fi

As a na\"{i}ve solution, for a %given 
\smash{$(q, d)$} pair, one can simply match a joint transformation of the student's query embedding \smash{${\tt emb}^{\rm s}_q$} and document embedding ${\tt emb}^{\rm s}_d$ to the teacher's joint embedding ${\tt emb}^{\rm t}_{q, d}$ , produced by (single) teacher encoder \smash{${\rm Enc}^{t}$}. % = {\rm pool}\big({\rm Enc}^{\rm t}(\tilde{o})\big)$. % produced by the teacher CE model. 
%
% Formally, this amounts to including the following to the training objective:
% \begin{equation}
%     \resizebox{.8\hsize}{!}{$\frac{1}{n}\sum\limits_{(q, d) \in \SCal_n} \| {\tt emb}^{\rm t}_{q, d} - {\rm mlp}\big({\tt emb}^{\rm s}_q, {\tt emb}^{\rm s}_d\big)\|$},\label{eq:emb-loss-ca2de-joint}
% \end{equation}
%where ${\rm mlp}$ is a trainable layer that maps the student query and document embeddings to the joint embedding space of the teacher. 
However, {we observed} that including such an embedding matching task often leads to severe over-fitting, and results in a poor student. 
Since
$
s^{\rm t}(q, d) = \langle w, {\tt emb}^{\rm t}_{q, d}\rangle
$, during CE model training, the joint embeddings ${\tt emb}^{\rm t}_{q, d}$ for relevant and irrelevant $(q, d)$ pairs are encouraged to be aligned with $w$ and $-w$, respectively. %; and the joint embeddings for irrelevant pairs are trained to align with $-w$.
{This produces degenerate embeddings that do not capture semantic query-to-document relationships. We notice that even the final query and document token embeddings lose such semantic structure (cf.~Appendix~\ref{appen:embed-analysis-ce2de}). Thus, a teacher CE model % trained 
with $s^{\rm t}(q, d) = \langle w, {\tt emb}^{\rm t}_{q, d}\rangle$ 
does not add value for distillation beyond score-matching;
in fact, it \emph{hurts} to include na\"{i}ve embedding matching.}
Next, we propose a modified CE model training strategy that facilitates %utilizing 
%distillation to DE models with embedding matching.
\embd.
%\vspace{1,5mm}

% Recall that the CE model relevance score typically takes the form
% $
% s^{\rm t}(q, d) = \langle w, {\tt emb}^{\rm t}_{q, d}\rangle.
% $ 
% Thus, during CE model training, the joint embedding ${\tt emb}^{\rm t}_{q, d}$ for relevant query-document pairs is encourage to be aligned along the single classification vector $w$; and the joint embedding for irrelevant pairs is trained to be aligned to $-w$. {This produces degenerate embeddings that do not capture semantic query-to-query and document-to-document relationships. In fact, we observed that even the final CE model query and document token embeddings lose such semantic structure. Thus, a teacher CE model trained with relevance scores $s^{\rm t}(q, d) = \langle w, {\tt emb}^{\rm t}_{q, d}\rangle$ does not add value beyond simple score-matching;
% in fact, it \emph{hurts} to include the above na\"{i}ve embedding-matching loss.}


% \begin{figure}
%     \centering
%     \includegraphics[page=4,width=0.6\linewidth,trim=0 6cm 8cm 0,clip]{figures/TGT-Beyond Drawing.pdf}
%     \caption{Embedding matching-based CE to DE distillation, with CE model employing dual pooling. % (cf.~Sec.~\ref{sec:cetode}). %Sec.~\ref{sec:cetode}. 
%     % {We employ a CE model with dual pooling as per Sec.~\ref{sec:cetode}.}
%     } %{\color{red} special token-based dual pooling (q.~\eqref{eq:special-dual-pooling} in Appendix~\ref{appendix:pooling})} to facilitate embedding alignment between the teacher and student, as per Sec.~\ref{sec:cetode}.}
%     \label{fig:ce2de-embed}
%     \vspace{-1em}
% \end{figure}

\noindent \textbf{CE models with dual pooling.}
% \sout{We \sout{propose}{\color{red}utilize} \emph{dual pooling}~\citep{yadav2022efficient}}
% \manzil{
A \emph{dual pooling} scheme is employed in the scoring layer
to produce two embeddings ${\tt emb}^{\rm t}_{q \leftarrow (q,d)}$ and ${\tt emb}^{\rm t}_{d \leftarrow (q,d)}$ from a CE model that serve as the \emph{proxy} query and document embeddings, respectively.
% ${\tt emb}^{\rm t}_{q \leftarrow (q,d)}$ and ${\tt emb}^{\rm t}_{d \leftarrow (q,d)}$. 
Accordingly, we define the relevance score 
%computed as the inner product between the two pooled embeddings, i.e., 
as $s^{\rm t}(q, d) = \langle {\tt emb}^{\rm t}_{q \leftarrow (q,d)},{\tt emb}^{\rm t}_{d \leftarrow (q,d)}\rangle$. We explore two variants of dual pooling: {(1) special token-based pooling that pools from \texttt{[CLS]} and \texttt{[SEP]}; and (2) segment-based weighted mean pooling that separately performs weighted averaging on the query and document segments of the final token embeddings. See Appendix~\ref{appendix:pooling} for details.}
% Instead of pooling a single embedding from the CA model, we propose \emph{dual pooling} that produces two embeddings from that serve as the \emph{proxy} query and document embeddings ${\tt emb}^{\rm t}_{q \leftarrow (q,d)}$ and ${\tt emb}^{\rm t}_{d \leftarrow (q,d)}$. The relevance score is then computed as the inner product between the two pooled embeddings, i.e., $s^{\rm t}(q, d) = \langle {\tt emb}^{\rm t}_{q \leftarrow (q,d)},{\tt emb}^{\rm t}_{d \leftarrow (q,d)}\rangle$. In particular, we explore two variants of dual pooling: \textcolor{red}{(1) special token-based pooling that pools from \texttt{[CLS]} and \texttt{[SEP]} (2) segment-based weighted mean pooling that takes weighted averaging on each query and document segment. Detailed formulations are in Appendix~\ref{appendix:pooling}.}

% Moved to Appendix.

% \begin{wrapfigure}{r}{0.55\linewidth}
%     \vspace{0mm}
%     \centering
%     \includegraphics[page=4,width=0.99\linewidth,trim=0 6.3cm 8cm 0,clip]{figures/TGT-Beyond Drawing.pdf}
%     % \vspace{-2mm}
%     \caption{Illustration of CE to DE distillation using \embd, with CE model employing dual pooling.}
%     \label{fig:ce2de-embed}
%     \vspace{-3mm}
% \end{wrapfigure}

In addition to %employing the 
dual pooling, we also utilize a reconstruction loss during the CE training, which measures the likelihood of predicting each token of the original input from the final %Transformer 
token embeddings. This loss encourages reconstruction of query and document tokens based on the final token embeddings and prevents the degeneration of the token embeddings during training. % on the IR task. 
%
%(cf.~Sec.~\ref{sec:bg}). 
%
%
Given proxy embeddings from the teacher CE, we can perform \embd~with %employ previously defined embedding matching loss in 
%\todoam{Fix eqref.}
the embedding matching loss defined in Eq.~\eqref{eq:emb-loss-de2de-q} and Eq.~\eqref{eq:emb-loss-de2de-d} %using the proxy embeddings 
(cf.~Fig.~\ref{fig:ce2de-embed}).
%$R_{\rm Emb}({\rm t}, {\rm s}; \SCal_n) = \sum_{(q, d) \in \SCal_n} \big[ \|{\tt emb}^{\rm t}_{q \leftarrow (q,d)}  - {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \|] + \|{\tt emb}^{\rm t}_{d \leftarrow (q,d)} - {\rm proj}\big({\tt emb}^{\rm s}_d) \| \big]/n$ 
%, which aims to align proxy query and document embeddings from the teacher CE model to the query and documents embeddings of the student DE model (cf.~Fig.~\ref{fig:ce2de-embed}).
% \begin{align}
% \label{eq:emb-loss-ca2de}
% \hspace{-2mm}
% % &R_{\tt emb}({\tt emb}^{\rm t}; {\tt emb}^{\rm s}) 
% R_{\rm Emb}({\rm t}, {\rm s}; \SCal_n) &= 
% %\nonumber \\ %\frac{1}{n}
% \sum_{(q, d) \in \SCal_n} \Big( 
% \|{\tt emb}^{\rm t}_{q \leftarrow (q,d)}  - {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \| \nonumber \\
% % \sum_{(q, d) \in \SCal_n} \Big(  \|{\tt emb}^{\rm t}_{q \leftarrow (q,d)}  - {\rm proj}\big({\tt emb}^{\rm s}_{q}\big) \| \nonumber \\
% &\;\;+ %\frac{1}{n}\sum_{d \in \SCal_n}
% \|{\tt emb}^{\rm t}_{d \leftarrow (q,d)} - {\rm proj}\big({\tt emb}^{\rm s}_d) \| \Big)/n,
% \end{align}
%where ${\rm proj}$ is an (optional) trainable layer that might be needed to match the embedding sizes.

